SkillAggregation: Reference-free LLM-Dependent Aggregation

Large Language Models (LLMs) are increasingly used to assess NLP tasks due to their ability to generate human-like judgments. Single LLMs were used initially, however, recent work suggests using multiple LLMs as judges yields improved performance. An important step in exploiting multiple judgements is the combination stage, aggregation. Existing methods in NLP either assign equal weight to all LLM judgments or are designed for specific tasks such as hallucination detection. This work focuses on aggregating predictions from multiple systems where no reference labels are available. A new method called SkillAggregation is proposed, which learns to combine estimates from LLM judges without needing additional data or ground truth. It extends the Crowdlayer aggregation method, developed for image classification, to exploit the judge estimates during inference. The approach is compared to a range of standard aggregation methods on HaluEval-Dialogue, TruthfulQA and Chatbot Arena tasks. SkillAggregation outperforms Crowdlayer on all tasks, and yields the best performance over all approaches on the majority of tasks.

==> scratch/scratch_intro.tex <==
\item llm as a judge
    \begin{itemize}
        \item humans are expensive -- how expensive? (10 mins x 25000 examples x 12/60 = 50000); (1000 tokens x 25000 examples x 5/1000000 = 125)
        \item On multiple datasets, it has been shown that using a ``strong" llm as a judge correlates with how humans give feedback.
        \item For example, \citet{li2024crowdsourced} collected a dataset that they call Arena-Hard-Auto v0.1. They take the rankings of LLMs on Chatbot Arena's overall leaderboard as ground truth and compare these with rankings produced by GPT-4 as a judge. On the first twenty top-ranked models, they obtain a Spearman correlation of 0.941.
        % \item On a dataset called Chatbot Arena Hard v0.1 CITE, take the rankings of 
    \end{itemize}


    \begin{itemize}
        \item higher correlation with human judgments
        \item \citet{verga2024replacing} take the rankings of LLMs on Chatbot Arena overall leaderboard as ground truth and compare these with rankings produced by GPT-4 as a judge and those produced by a panel of LLMs. Spearman correlation increases from 0.817 to 0.917.
        \item \citet{li2023prd} take the Vicuna80 dataset and improve the accuracy by 0.6\% over Majority Vote.
    \end{itemize}
